Anchor-free Oriented Proposal Generator for Object Detection

Oriented object detection is a practical and challenging task in remote sensing image interpretation. Nowadays, oriented detectors mostly use horizontal boxes as intermedium to derive oriented boxes from them. However, the horizontal boxes are inclined to get small Intersection-over-Unions (IoUs) with ground truths, which may have some undesirable effects, such as introducing redundant noise, mismatching with ground truths, detracting from the robustness of detectors, etc. In this paper, we propose a novel Anchor-free Oriented Proposal Generator (AOPG) that abandons horizontal box-related operations from the network architecture. AOPG first produces coarse oriented boxes by a Coarse Location Module (CLM) in an anchor-free manner and then refines them into high-quality oriented proposals. After AOPG, we apply a Fast R-CNN head to produce the final detection results. Furthermore, the shortage of large-scale datasets is also a hindrance to the development of oriented object detection. To alleviate the data insufficiency, we release a new dataset on the basis of our DIOR dataset and name it DIOR-R. Massive experiments demonstrate the effectiveness of AOPG. Particularly, without bells and whistles, we achieve the accuracy of 64.41%, 75.24% and 96.22% mAP on the DIOR-R, DOTA and HRSC2016 datasets respectively. Code and models are available at https://github.com/jbwang1997/AOPG.

==> 6-biography.tex <==
\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{pic/cg.jpg}}]
{Gong Cheng} received the B.S. degree from Xidian University, Xi’an, China, in 2007, and the M.S. and Ph.D. degrees from Northwestern Polytechnical University, Xi’an, in 2010 and 2013, respectively.

He is a Professor with Northwestern Polytechnical University. His main research interests are computer vision, pattern recognition, and remote sensing image understanding.

Dr. Cheng is an Associate Editor of \textit{IEEE Geoscience and Remote Sensing Magazine} and a Guest Editor of IEEE Journal of Selected Topics in Applied Earth Observations and Remote Sensing.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{pic/wjb.jpg}}]
{Jiabao Wang}
received the B.S. degree from Northwestern Polytechnical University, Xi’an, China, in 2019. 

He is currently pursuing the master’s degree at Northwestern Polytechnical University, Xi’an, China.
His research interests include computer vision and pattern recognition, especially object detection.
\end{IEEEbiography}



\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{pic/lk.jpg}}]
{Ke Li}
received the M.Sc. and Ph.D. degrees from the Zhengzhou Institute of Surveying and Mapping, Zhengzhou, China, in 2005 and 2008, respectively.

He is currently an Associate Professor with the Zhengzhou Institute of Surveying and Mapping. His research interests include geographic information system, deep learning, and remote sensing image analysis.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{pic/xxx.jpg}}]
{Xingxing Xie}
received the B.S. degree from Inner Mongolia University, Huhhot, China, in 2015, and the M.S. degree from Northwestern Polytechnical University, Xi'an, China, in 2018.

He is currently pursuing the Ph.D degree at Northwestern Polytechnical University. His main research interests are computer vision and pattern recognition. 
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{pic/lcb.jpg}}]
{Chunbo Lang}
Chunbo Lang received the B.Eng. degree from Northeast Forestry University, Harbin, China, in 2020. 

He is currently a 2nd year Ph.D. student in Northwestern Polytechnical University, Xi'an, China, under the supervision of Prof. Gong Cheng. His research interests include few-shot learning, segmentation, and remote sensing image understanding.
\end{IEEEbiography}


\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{pic/yyq.jpg}}]
{Yanqing Yao}
received the B.S. and M.S., degrees from Inner Mongolia University of Science and Technology, Baotou, China, in 2016 and 2019, respectively. 

She is currently pursuing the Ph.D degree at Northwestern Polytechnical University. Her research interests include computer vision and image processing, especially on remote sensing image analysis.
\end{IEEEbiography}





\begin{IEEEbiography}
[{\includegraphics[width=1in, height=1.25in,clip,keepaspectratio]{pic/hjw.jpg}}]
{Junwei Han}
received the B.S., M.S., and Ph.D. degrees in pattern recognition and intelligent systems from Northwestern Polytechnical University, Xi’an, China, in 1999, 2001, and 2003, respectively.

He was a Research Fellow with Nanyang Technological University, Singapore, The Chinese University of Hong Kong, Hong Kong, the Dublin City University, Dublin, Ireland, and the University of Dundee, Dundee, U.K., from 2003 to 2010. He is a Professor with Northwestern Polytechnical University. His research interests include computer vision
and brain imaging analysis. He is a fellow of the IEEE.



\end{IEEEbiography}

==> temp.tex <==
To illustrate the aforementioned problems, we show the occasion that both horizontal and oriented proposals are assigned with the same ground truth in Figure~\ref{img:issues}. As we can see. (i) The horizontal proposal includes at least four vehicles. Thus, it is very difficult for detectors to precisely classify and localize the targets. (ii) Even the horizontal proposal has been assigned as positive, it only presents a small IoU of 0.16 with the ground truth. In contrast, the oriented proposal has a big IoU of 0.87. (iii) The regression target from the horizontal proposal to the ground truth reaches 2.06, which is very large for training detectors. As shown in the right figure, the regression target of the oriented proposal is just 0.14, which is much smaller than the horizontal proposal.


RoI Transformer~\cite{ding2019} attempts to train a lightweight module, named rotated RoI learner, to predict oriented proposals from horizontal proposals. The rotated RoI learner is flexible to plug in all two-stage detectors and largely increases the detection accuracy. Nevertheless, there still leave some horizontal parts in RoI Transformer. For example, RoI Transformer uses horizontal proposals to recall the oriented objects, which suffers from the same disadvantages as other detectors with horizontal schemes. Besides, the recent official RoI Transformer abolishes the lightweight design of RoI learner to achieve higher results, making RoI Transformer much more inefficient.

targeting to generate high-quality oriented proposals but without involving horizontal boxes.


In the aspect of aerial image interpretation, DABNet~\cite{9314019} enhances the features by taking advantage of the deformable context feature pyramid module to achieve high-accuracy detection of complex clouds. ~\cite{9328476}






\begin{table*}\small
	%\setlength{\abovecaptionskip}{0.2cm}
	\setlength{\belowcaptionskip}{-1cm}
	\renewcommand\arraystretch{1.5}
	\caption{Comparison with state-of-the-art methods on the DOTA dataset. * means the results from AerialDetection (the same below). $^\ddagger$ denotes multi-scale training and testing.}
	\label{table:dota_comparison}
	\begin{center}
		\resizebox{1.0\textwidth}{!}{
			\begin{tabular}{p{3cm}<{\centering}|p{2.5cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}|p{0.8cm}<{\centering}}
				\hline
				Method                      & Backbone  & PL             & BD             & BR             & GTF            & SV             & LV             & SH             & TC             & BC             & ST             & SBF            & RA             & HA             & SP             & HC             & mAP            \\ \hline
				\textit{\textbf{One-stage}} & \multicolumn{17}{c}{}                                                                                                                                                                                                                                                                    \\ \hline
				PIoU~\cite{chen2020piou}                        & DLA-34    & 80.90          & 69.70          & 24.10          & 60.20          & 38.30          & 64.40          & 64.80          & \textbf{90.90} & 77.20          & 70.40          & 46.50          & 37.10          & 57.10          & 61.90          & 64.00          & 60.50          \\
				RetinaNet-O*~\cite{lin2017focal}              & R-50-FPN  & 88.67          & 77.62          & 41.81          & 58.17          & 74.58          & 71.64          & 79.11          & 90.29          & 82.18          & 74.32          & 54.75          & 60.60          & 62.57          & 69.67          & 60.64          & 68.43          \\
				DRN~\cite{pan2020dynamic}                         & H-104     & 88.91          & 80.22          & 43.52          & 63.35          & 73.48          & 70.69          & 84.94          & 90.14          & 83.85          & 84.11          & 50.12          & 58.41          & 67.62          & 68.60          & 52.50          & 70.70          \\ 
				DAL~\cite{ming2020dynamic}                         & R-50-FPN  & 88.68          & 76.55          & 45.08          & 66.80          & 67.00          & 76.76          & 79.74          & 90.84          & 79.54          & 78.45          & 57.71          & 62.27          & 69.05          & 73.14          & 60.11          & 71.44          \\ 
				RSDet~\cite{qian2019learning}                       & R-101-FPN & 89.80          & 82.90          & 48.60          & 65.20          & 69.50          & 70.10          & 70.20          & 90.50          & 85.60          & 83.40          & 62.50          & 63.90          & 65.60          & 67.20          & 68.00          & 72.20          \\ 
				R3Det~\cite{yang2019r3det}                       & R-101-FPN & 88.76          & 83.09          & 50.91          & 67.27          & 76.23          & 80.39          & 86.72          & 90.78          & 84.68          & 83.24          & 61.98          & 61.35          & 66.91          & 70.63          & 53.94          & 73.79          \\ 
				S$^2$ANet~\cite{han2021}                      & R-50-FPN  & 89.11          & 82.84          & 48.37          & 71.11          & 78.11          & 78.39          & 87.25          & 90.83          & 84.90          & 85.64          & 60.36          & 62.60          & 65.26          & 69.13          & 57.94          & 74.12          \\ \hline
				\textit{\textbf{Two-stage}} & \multicolumn{17}{c}{}                                                                                                                                                                                                                                                                    \\ \hline
				RRPN~\cite{ma2018}                        & R-101     & 80.94          & 65.75          & 35.34          & 67.44          & 59.92          & 50.91          & 55.81          & 90.67          & 66.92          & 72.39          & 55.06          & 52.23          & 55.14          & 53.35          & 48.22          & 60.01          \\ 
				R2CN~\cite{jiang2017r2cnn}                       & R-101     & 80.94          & 65.67          & 35.34          & 67.44          & 59.92          & 50.91          & 55.81          & 90.67          & 66.92          & 72.39          & 55.06          & 52.23          & 55.14          & 53.35          & 48.22          & 60.67          \\ 
				RoI Transformer~\cite{ding2019}             & R-101-FPN & 88.64          & 78.52          & 43.44          & 75.92          & 68.81          & 73.68          & 83.59          & 90.74          & 77.27          & 81.46          & 58.39          & 53.54          & 62.83          & 58.93          & 47.67          & 69.56          \\ 
				SCRDet~\cite{yang2019}                      & R-101-FPN & \textbf{89.98} & 80.65          & 52.09          & 68.36          & 68.36          & 60.32          & 72.41          & 90.85          & \textbf{87.94} & 86.86          & 65.02          & 66.68          & 66.25          & 68.24          & 65.21          & 72.61          \\ 
				RoI Transformer*~\cite{ding2019}            & R-50-FPN  & 88.65          & 82.60          & 52.53          & 70.87          & 77.93          & 76.67          & 86.87          & 90.71          & 83.83          & 82.51          & 53.95          & 67.61          & 74.67          & 68.75          & 61.03          & 74.61          \\ 
				Gliding Vertex~\cite{xu2020}             & R-101-FPN & 89.64          & 85.00          & 52.26          & 77.34          & 73.01          & 73.14          & 86.82          & 90.74          & 79.02          & 86.81          & 59.55          & 70.91          & 72.94          & 70.86          & 57.32          & 75.02          \\ 
				Faster RCNN-O*~\cite{ren2016}           & R-50-FPN  & 88.44          & 73.06          & 44.86          & 59.09          & 73.25          & 71.49          & 77.11          & 90.84          & 78.94          & 83.90          & 48.59          & 62.95          & 62.18          & 64.91          & 56.18          & 69.05          \\  \hline
				\textit{\textbf{Ours}} & \multicolumn{17}{c}{}                                                                                                                                                                                                                                                                    \\ \hline
				AOPG                   & R-50-FPN  & 89.27          & 83.49          & 52.50          & 69.97          & 73.51          & 82.31          & 87.95          & 90.89          & 87.64          & 84.71          & 60.01          & 66.12          & 74.19          & 68.30          & 57.80          & 75.24          \\ 
				AOPG                    & R-101-FPN & 89.14          & 82.74          & 51.87          & 69.28          & 77.65          & 82.42          & 88.08          & 90.89          & 86.26          & 85.13          & 60.60          & 66.30          & 74.05          & 67.76          & 58.77          & 75.39          \\ 
				AOPG$^\ddagger$                   & R-50-FPN  & 89.88          & 85.57          & \textbf{60.90} & \textbf{81.51} & \textbf{78.70} & \textbf{85.29} & \textbf{88.85} & 90.89          & 87.60          & \textbf{87.65} & \textbf{71.66} & 68.69          & 82.31          & \textbf{77.32} & \textbf{73.10} & \textbf{80.66} \\ 
				AOPG$^\ddagger$                  & R-101-FPN & \textbf{89.98} & \textbf{86.14} & 60.20          & 79.55          & 78.47          & 84.93          & 88.79          & 90.88          & 87.32          & 87.07          & 71.50          & \textbf{71.22} & \textbf{83.57} & 72.47          & 70.77          & 80.19          \\ \hline
		\end{tabular}}
	\end{center}
%	\vspace*{-4mm}
%	\vspace{0.6\baselineskip}
\end{table*}

